The Hidden Bias of Process Reward Models:PRISM for Rewarding the Right Reasoning

Process Reward Models (PRMs) improve credit assignment for reasoning by providing step-level feedback. However, we identify a hidden bias in PRMs caused by severe imbalance in step-level training data. Standard cross-entropy training amplifies this bias, causing PRMs to overcredit plausible but incorrect steps and produce high false-positive rates. We show that these false positives have an asymmetric downstream effect: false negatives mainly slow exploration, whereas false positives actively steer Best-of-N selection, guided decoding, and policy optimization toward flawed reasoning. This suggests that PRM training should shift from pointwise label fitting to reliable relative comparisons. To address this, we propose PRISM (Precision Ranking for Improved Step Modeling), a policy-aware PRM training framework that learns from contrastive step-level comparisons and hard negatives generated by a temporal lookahead strategy, requiring no new human labels. We further use a difficulty-aware curriculum to optimize the contrastive step margin. Across PRMBench and ProcessBench, PRISM substantially reduces false positives (22% on PRMBench) and improves macro F1 over strong discriminative PRMs. When applied to policy optimization and search tasks, including guided decoding and Best-of-N selection, it consistently improves accuracy (up to 22% for guided decoding and 33% for Best-of-N) and robustness. More broadly, trustworthy process supervision is not just about assigning high rewards, but about rewarding the right reasoning for the right reasons.

==> Figures/teaser_aak_old.tex <==
\begin{tikzpicture}[x=1cm,y=1cm, >=Latex, font=\sffamily]
    % --- Premium Color Palette ---
    \definecolor{primary}{RGB}{31,59,91}       % Deep Navy
    \definecolor{accent}{RGB}{52, 101, 164}    % Soft Blue
    \definecolor{good}{RGB}{46, 139, 87}       % Sea Green
    \definecolor{bad}{RGB}{205, 92, 92}        % Indian Red
    \definecolor{bglight}{RGB}{248, 249, 250}  % Off-white for panels
    \definecolor{boxborder}{RGB}{222, 226, 230}% Soft gray for borders
    \definecolor{subtext}{RGB}{80, 80, 80}     % Dark gray for subtext
    
    % --- Global Styles ---
    \tikzstyle{panel} = [draw=boxborder, fill=bglight, rounded corners=2mm, inner sep=0pt]
    \tikzstyle{header} = [font=\bfseries, text=primary, anchor=north west]
    \tikzstyle{subtext} = [font=\scriptsize, text=subtext, align=left, anchor=north west]
    \tikzstyle{nodebox} = [draw=boxborder, fill=white, rounded corners=1mm, align=center, font=\scriptsize, inner sep=1.5mm]
    \tikzstyle{pill} = [rounded corners=1.5mm, inner xsep=1.5mm, inner ysep=1mm, font=\tiny\bfseries, align=center]
    
    % ==========================================
    % TOP BANNER
    % ==========================================
    \node[fill=primary, text=white, rounded corners=1.5mm, minimum width=17.8cm, minimum height=0.7cm, font=\bfseries] at (8.9, 5.3) {PRISM Reduces False--Positives In Process Rewards Models For Better Policy Learning.};

    % ==========================================
    % PANEL 1: DIAGNOSE THE FAILURE MODE
    % ==========================================
    \node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p1) at (0, 0) {};
    \node[header] at (0.2, 4.3) {1. The Failure Mode};
    \node[subtext, text width=5.2cm] at (0.2, 3.8) {PRM overcredits plausible mistake steps, creating an alignment ceiling.};
    
    % Boxes
    % \node[nodebox, draw=good, fill=good!5, text width=3.4cm, anchor=north west] (p1_good) at (0.2, 2.8) {\textbf{Correct Continuation}\\[0.5mm] $DF=10$, then solve for $DE$.};
    % \node[nodebox, draw=bad, fill=bad!5, text width=3.4cm, anchor=north west] (p1_bad) at (0.2, 1.5) {\textbf{Plausible but Wrong}\\[0.5mm] Uses $DE$ instead of $DF$.};
    % Boxes
    \node[nodebox, draw=good, fill=good!5, text width=3.4cm, anchor=north west] (p1_good) at (0.2, 2.8) {\textbf{Correct Continuation}\\[0.5mm] $(x+2)^2 = 9 \implies x+2 = \pm 3$};
    \node[nodebox, draw=bad, fill=bad!5, text width=3.4cm, anchor=north west] (p1_bad) at (0.2, 1.5) {\textbf{Plausible but Wrong}\\[0.5mm] $(x+2)^2 = 9 \implies x^2 + 4 = 9$};

    
    % Metrics (Styled as pills)
    \node[pill, fill=good!15, text=good, anchor=west] at (3.8, 2.3) {Reward $\uparrow$};
    \node[pill, fill=bad!15, text=bad, anchor=west] at (3.8, 1.1) {PRM: 0.91};
    \node[pill, fill=primary!15, text=primary, anchor=west] at (3.8, 0.5) {PRISM: 0.18};

    % ==========================================
    % PANEL 2: TRAIN FOR RELIABILITY
    % ==========================================
    \node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p2) at (6.05, 0) {};
    \node[header] at (6.25, 4.3) {2. PRISM Training};
    \node[subtext, text width=5.2cm] at (6.25, 3.8) {Optimize reward margin using contrastive training on hard negatives.};
    
    % Flow Nodes
    % \node[nodebox, text width=1.6cm, anchor=west] (ctx) at (6.25, 2.15) {\textbf{Prefix Context}\\$S(<t)$};
    % \node[nodebox, draw=good, text width=1.8cm, anchor=west] (pos) at (8.8, 2.8) {\textbf{Matched Pos.}\\$S(t)$};
    % \node[nodebox, draw=bad, text width=1.8cm, anchor=west] (neg) at (8.8, 1.5) {\textbf{Hard Neg.}\\$S(K)$};
    % \node[nodebox, draw=accent, fill=accent!10, text width=5cm, anchor=north] (loss) at (8.9, 0.8) {\textbf{Step--Contrastive Objective}\\+ Difficulty Curriculum};
    % Flow Nodes
    \node[nodebox, text width=1.6cm, anchor=west] (ctx) at (6.25, 2.15) {\textbf{Prefix Context}\\$x, s(<t)$};
    
    \node[nodebox, draw=good, line width=0.8pt, text width=1.8cm, anchor=west] (pos) at (8.8, 2.8) {\textbf{Positive Step}\\$s(t)$};
    \node[circle, fill=good, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]pos.north west) {1};
    
    \node[nodebox, draw=bad, line width=0.8pt, text width=1.8cm, anchor=west] (neg) at (8.8, 1.5) {\textbf{Hard Neg. Step}\\$s(>t)$};
    \node[circle, fill=bad, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]neg.north west) {2};
    
    \node[nodebox, draw=accent, line width=0.8pt, fill=accent!10, text width=5cm, anchor=north] (loss) at (8.9, 0.8) {\textbf{Step--Contrastive Loss}\\+ Margin Aware Difficulty Curriculum};
    \node[circle, fill=accent, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]loss.north west) {3};
    
 % Connecting Arrows
    % \draw[->, primary, thick] (ctx.east) to[out=0, in=180] (pos.west);
    % \draw[->, primary, thick] (ctx.east) to[out=0, in=180] (neg.west);
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.2,0) |- (pos.west);
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.2,0) |- (neg.west);
    \draw[->, accent, thick, rounded corners] (pos.east) -| ([xshift=2.4cm]loss.north);
    \draw[->, accent, thick, rounded corners] (neg.east) -| ([xshift=2.2cm]loss.north);

    % ==========================================
    % PANEL 3: GAIN DOWNSTREAM IMPACT
    % ==========================================
\node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p3) at (12.1, 0) {};
    \node[header] at (12.3, 4.3) {3. Downstream Impact};
    \node[subtext, text width=5.2cm] at (12.3, 3.8) {Higher precision translates into safer ranking and guided search.};
    
    % FPR Callout Badge
    \node[nodebox, draw=none, fill=accent!15, anchor=north, font=\scriptsize] at (14.95, 3.0) {\textbf{PRM's FPR}: $\mathbf{69.3 \% \rightarrow 47.1\%}$};

    % Custom TikZ Graph (Clean and precise)
    \begin{scope}[shift={(13.0, 0.6)}]
        % Grid and Axes
        \draw[lightgray, very thin, dashed] (0,0) -- (3.9,0);
        \draw[lightgray, very thin, dashed] (0,0.3) -- (3.9,0.3);
        \draw[lightgray, very thin, dashed] (0,0.6) -- (3.9,0.6);
        \draw[lightgray, very thin, dashed] (0,0.9) -- (3.9,0.9);
        \draw[lightgray, very thin, dashed] (0,1.2) -- (3.9,1.2);
        \draw[lightgray, very thin, dashed] (0,1.5) -- (3.9,1.5);
        \draw[lightgray, very thin, dashed] (0,1.8) -- (3.9,1.8);
        
        \draw[->, darkgray, thick] (0,0) -- (0,2.0) node[left, font=\tiny, rotate=90, yshift=2mm, xshift=-6mm] {AIME '24 Acc. (\%)};
        
        % Baseline Line (Orange/bad - PRM)
        \draw[bad, thick, densely dashed] (0,0.1) -- (0.65,0.1) -- (1.3,0.1) -- (1.95,0.1) -- (2.6,0.1) -- (3.25,0.6) -- (3.9,0.6);
        \fill[bad] (0,0.1) circle (1.2pt) (0.65,0.1) circle (1.2pt) (1.3,0.1) circle (1.2pt) (1.95,0.1) circle (1.2pt) (2.6,0.1) circle (1.2pt) (3.25,0.6) circle (1.2pt) (3.9,0.6) circle (1.2pt);
        
        % PRISM Line (Green/good - Ours)
        \draw[good, thick] (0,0.6) -- (0.65,0.6) -- (1.3,0.6) -- (1.95,0.6) -- (2.6,1.1) -- (3.25,1.6) -- (3.9,1.6);
        \fill[good] (0,0.6) circle (1.2pt) (0.65,0.6) circle (1.2pt) (1.3,0.6) circle (1.2pt) (1.95,0.6) circle (1.2pt) (2.6,1.1) circle (1.2pt) (3.25,1.6) circle (1.2pt) (3.9,1.6) circle (1.2pt);
        
        % Legend labels
        \node[font=\tiny\bfseries, text=bad, anchor=south] at (2.2, 0.15) {PRM}; % Shifted slightly above the bad line
        \node[font=\tiny\bfseries, text=good, anchor=south east] at (3.3, 1.65) {PRISM};

        % X-axis Labels (Shifted closer to the axis using inner sep=2pt and y=0)
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (0,0) {$2^0$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (0.65,0) {$2^1$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (1.3,0) {$2^2$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (1.95,0) {$2^3$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (2.6,0) {$2^4$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (3.25,0) {$2^5$};
        \node[font=\tiny, text=darkgray, anchor=north, inner sep=2pt] at (3.9,0) {$2^6$};
        
        % X-axis Title
        \node[font=\tiny, text=darkgray, anchor=north] at (1.95, -0.3) {No. of Solutions};
    \end{scope}

    % ==========================================
    % INTER-PANEL ARROWS
    % ==========================================
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (5.75, 2.25) -- (6.0, 2.25);
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (11.8, 2.25) -- (12.05, 2.25);
\end{tikzpicture}

==> Figures/teaser_figure_v3.tex <==
\begin{tikzpicture}[x=1cm,y=1cm, >=Latex, font=\sffamily]
    % --- Premium Color Palette ---
    \definecolor{primary}{RGB}{31,59,91}       % Deep Navy
    \definecolor{accent}{RGB}{52, 101, 164}    % Soft Blue
    \definecolor{good}{RGB}{46, 139, 87}       % Sea Green
    \definecolor{bad}{RGB}{205, 92, 92}        % Indian Red
    \definecolor{bglight}{RGB}{248, 249, 250}  % Off-white for panels
    \definecolor{boxborder}{RGB}{222, 226, 230}% Soft gray for borders
    
    % --- Global Styles ---
    \tikzstyle{panel} = [draw=boxborder, fill=bglight, rounded corners=2mm, inner sep=0pt]
    \tikzstyle{header} = [font=\bfseries, text=primary, anchor=north west]
    \tikzstyle{subtext} = [font=\scriptsize, text=darkgray, align=left]
    \tikzstyle{nodebox} = [draw=boxborder, fill=white, rounded corners=1mm, align=center, font=\scriptsize, inner sep=1.5mm]
    
    % ==========================================
    % TOP BANNER: The Core Contribution
    % ==========================================
    \node[fill=primary, text=white, rounded corners=1.5mm, minimum width=17.4cm, minimum height=0.8cm, font=\small\bfseries] at (8.7, 5.5) {PRISM reduces false--positive overcredit so process rewards track sound reasoning instead of plausible mistakes.};

    % ==========================================
    % PANEL 1: DIAGNOSE THE FAILURE MODE
    % ==========================================
    \node[panel, minimum width=5.5cm, minimum height=4.5cm] (p1) at (2.75, 2.5) {};
    \node[header] at (0.2, 4.5) {1. The Failure Mode};
    \node[subtext, text width=5cm] at (0.2, 4.0) {Baselines overcredit plausible mistakes, creating an alignment ceiling.};
    
    \node[nodebox, draw=good, fill=good!5, text width=4.6cm, anchor=north] (p1_good) at (2.75, 3.3) {\textbf{Correct Continuation}\\$DF=10$, then solve for $DE$.};
    \node[nodebox, draw=bad, fill=bad!5, text width=4.6cm, anchor=north] (p1_bad) at (2.75, 2.1) {\textbf{Plausible but Wrong}\\Uses $DE$ instead of $DF$.};
    
    % Metrics inside Panel 1
    \node[font=\scriptsize\bfseries, text=good, anchor=east] at (4.9, 2.9) {Reward $\uparrow$};
    \node[font=\scriptsize\bfseries, text=bad, anchor=east] at (4.9, 1.85) {Baseline: 0.91};
    \node[font=\scriptsize\bfseries, text=primary, anchor=east] at (4.9, 1.45) {PRISM: 0.18};

    % ==========================================
    % PANEL 2: TRAIN FOR RELIABILITY
    % ==========================================
    \node[panel, minimum width=5.5cm, minimum height=4.5cm] (p2) at (8.7, 2.5) {};
    \node[header] at (6.15, 4.5) {2. PRISM Training};
    \node[subtext, text width=5cm] at (6.15, 4.0) {Optimize relative margins using temporal lookahead hard negatives.};
    
    \node[nodebox, text width=1.8cm, anchor=north] (ctx) at (7.3, 3.2) {\textbf{Prefix Context}\\$S(<t)$};
    \node[nodebox, draw=good, text width=1.8cm, anchor=north] (pos) at (10.2, 3.65) {\textbf{Matched Pos.}\\$S(t)$};
    \node[nodebox, draw=bad, text width=1.8cm, anchor=north] (neg) at (10.2, 2.5) {\textbf{Hard Neg.}\\$S(K)$};
    
    \node[nodebox, draw=accent, fill=accent!10, text width=4.8cm, anchor=north] (loss) at (8.7, 1.3) {\textbf{Step--Contrastive Objective}\\+ Difficulty Curriculum};
    
    % Connecting Arrows
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.3,0) |- (pos.west);
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.3,0) |- (neg.west);
    \draw[->, accent, thick] (pos.south) -- ++(0,-0.1) -| (loss.north);
    \draw[->, accent, thick] (neg.south) -- (neg.south |- loss.north);

    % ==========================================
    % PANEL 3: GAIN DOWNSTREAM IMPACT
    % ==========================================
    \node[panel, minimum width=5.5cm, minimum height=4.5cm] (p3) at (14.65, 2.5) {};
    \node[header] at (12.1, 4.5) {3. Downstream Impact};
    \node[subtext, text width=5cm] at (12.1, 4.0) {Higher precision translates into safer ranking and guided search.};
    
    % FPR Callout Badge
    \node[nodebox, draw=none, fill=accent!15, anchor=north] at (14.65, 3.4) {\textbf{PRMBench FPR}: $\mathbf{69.3 \rightarrow 47.1}$};

    % Stylized Custom TikZ Graph for perfect consistency
    \begin{scope}[shift={(12.6, 0.9)}]
        % Grid and Axes
        \draw[lightgray, very thin, dashed] (0,0) -- (3.5,0);
        \draw[lightgray, very thin, dashed] (0,0.7) -- (3.5,0.7);
        \draw[lightgray, very thin, dashed] (0,1.4) -- (3.5,1.4);
        \draw[->, darkgray, thick] (0,0) -- (3.8,0) node[below, font=\tiny, xshift=-15mm, yshift=-1mm] {Solutions ($2^k$)};
        \draw[->, darkgray, thick] (0,0) -- (0,1.8) node[left, font=\tiny, rotate=90, yshift=2mm, xshift=-6mm] {AIME '24 Acc.};
        
        % Baseline Line
        \draw[bad, thick, densely dashed] (0,0.1) -- (0.7,0.1) -- (1.4,0.1) -- (2.1,0.1) -- (2.8,0.4) -- (3.5,0.4);
        \fill[bad] (0,0.1) circle (1.2pt) (0.7,0.1) circle (1.2pt) (1.4,0.1) circle (1.2pt) (2.1,0.1) circle (1.2pt) (2.8,0.4) circle (1.2pt) (3.5,0.4) circle (1.2pt);
        
        % PRISM Line
        \draw[good, thick] (0,0.4) -- (0.7,0.4) -- (1.4,0.4) -- (2.1,0.4) -- (2.8,0.9) -- (3.5,1.5);
        \fill[good] (0,0.4) circle (1.2pt) (0.7,0.4) circle (1.2pt) (1.4,0.4) circle (1.2pt) (2.1,0.4) circle (1.2pt) (2.8,0.9) circle (1.2pt) (3.5,1.5) circle (1.2pt);
        
        % Legend labels
        \node[font=\tiny\bfseries, text=bad, anchor=west] at (3.6, 0.4) {Baseline};
        \node[font=\tiny\bfseries, text=good, anchor=west] at (3.6, 1.5) {PRISM};
    \end{scope}

    % ==========================================
    % INTER-PANEL ARROWS
    % ==========================================
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (5.5, 2.5) -- (5.95, 2.5);
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (11.45, 2.5) -- (11.9, 2.5);

\end{tikzpicture}

==> Figures/teaser_figure_v4.tex <==
\begin{tikzpicture}[x=1cm,y=1cm, >=Latex, font=\sffamily]
    % --- Premium Color Palette ---
    \definecolor{primary}{RGB}{31,59,91}       % Deep Navy
    \definecolor{accent}{RGB}{52, 101, 164}    % Soft Blue
    \definecolor{good}{RGB}{46, 139, 87}       % Sea Green
    \definecolor{bad}{RGB}{205, 92, 92}        % Indian Red
    \definecolor{bglight}{RGB}{248, 249, 250}  % Off-white for panels
    \definecolor{boxborder}{RGB}{222, 226, 230}% Soft gray for borders
    \definecolor{subtext}{RGB}{80, 80, 80}     % Dark gray for subtext
    
    % --- Global Styles ---
    \tikzstyle{panel} = [draw=boxborder, fill=bglight, rounded corners=2mm, inner sep=0pt]
    \tikzstyle{header} = [font=\bfseries, text=primary, anchor=north west]
    \tikzstyle{subtext} = [font=\scriptsize, text=subtext, align=left, anchor=north west]
    \tikzstyle{nodebox} = [draw=boxborder, fill=white, rounded corners=1mm, align=center, font=\scriptsize, inner sep=1.5mm]
    \tikzstyle{pill} = [rounded corners=1.5mm, inner xsep=1.5mm, inner ysep=1mm, font=\tiny\bfseries, align=center]
    
    % ==========================================
    % TOP BANNER
    % ==========================================
    \node[fill=primary, text=white, rounded corners=1.5mm, minimum width=17.8cm, minimum height=0.7cm, font=\small\bfseries] at (8.9, 5.3) {PRISM reduces false--positive overcredit so process rewards track sound reasoning instead of plausible mistakes.};

    % ==========================================
    % PANEL 1: DIAGNOSE THE FAILURE MODE
    % ==========================================
    \node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p1) at (0, 0) {};
    \node[header] at (0.2, 4.3) {1. The Failure Mode};
    \node[subtext, text width=5.2cm] at (0.2, 3.8) {PRM overcredits plausible mistake steps, creating an alignment ceiling.};
    
    % Boxes
    % \node[nodebox, draw=good, fill=good!5, text width=3.4cm, anchor=north west] (p1_good) at (0.2, 2.8) {\textbf{Correct Continuation}\\[0.5mm] $DF=10$, then solve for $DE$.};
    % \node[nodebox, draw=bad, fill=bad!5, text width=3.4cm, anchor=north west] (p1_bad) at (0.2, 1.5) {\textbf{Plausible but Wrong}\\[0.5mm] Uses $DE$ instead of $DF$.};
    % Boxes
    \node[nodebox, draw=good, fill=good!5, text width=3.4cm, anchor=north west] (p1_good) at (0.2, 2.8) {\textbf{Correct Continuation}\\[0.5mm] $(x+2)^2 = 9 \implies x+2 = \pm 3$};
    \node[nodebox, draw=bad, fill=bad!5, text width=3.4cm, anchor=north west] (p1_bad) at (0.2, 1.5) {\textbf{Plausible but Wrong}\\[0.5mm] $(x+2)^2 = 9 \implies x^2 + 4 = 9$};

    
    % Metrics (Styled as pills)
    \node[pill, fill=good!15, text=good, anchor=west] at (3.8, 2.3) {Reward $\uparrow$};
    \node[pill, fill=bad!15, text=bad, anchor=west] at (3.8, 1.1) {PRM: 0.91};
    \node[pill, fill=primary!15, text=primary, anchor=west] at (3.8, 0.5) {PRISM: 0.18};

    % ==========================================
    % PANEL 2: TRAIN FOR RELIABILITY
    % ==========================================
    \node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p2) at (6.05, 0) {};
    \node[header] at (6.25, 4.3) {2. PRISM Training};
    \node[subtext, text width=5.2cm] at (6.25, 3.8) {Optimize relative margins using temporal lookahead hard negatives.};
    
    % Flow Nodes
    % \node[nodebox, text width=1.6cm, anchor=west] (ctx) at (6.25, 2.15) {\textbf{Prefix Context}\\$S(<t)$};
    % \node[nodebox, draw=good, text width=1.8cm, anchor=west] (pos) at (8.8, 2.8) {\textbf{Matched Pos.}\\$S(t)$};
    % \node[nodebox, draw=bad, text width=1.8cm, anchor=west] (neg) at (8.8, 1.5) {\textbf{Hard Neg.}\\$S(K)$};
    % \node[nodebox, draw=accent, fill=accent!10, text width=5cm, anchor=north] (loss) at (8.9, 0.8) {\textbf{Step--Contrastive Objective}\\+ Difficulty Curriculum};
    % Flow Nodes
    \node[nodebox, text width=1.6cm, anchor=west] (ctx) at (6.25, 2.15) {\textbf{Prefix Context}\\$S(<t)$};
    
    \node[nodebox, draw=good, line width=0.8pt, text width=1.8cm, anchor=west] (pos) at (8.8, 2.8) {\textbf{Matched Pos.}\\$S(t)$};
    \node[circle, fill=good, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]pos.north west) {1};
    
    \node[nodebox, draw=bad, line width=0.8pt, text width=1.8cm, anchor=west] (neg) at (8.8, 1.5) {\textbf{Hard Neg.}\\$S(K_{>t})$};
    \node[circle, fill=bad, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]neg.north west) {2};
    
    \node[nodebox, draw=accent, line width=0.8pt, fill=accent!10, text width=5cm, anchor=north] (loss) at (8.9, 0.8) {\textbf{Step--Contrastive Obj.}\\+ Difficulty Curriculum};
    \node[circle, fill=accent, text=white, font=\tiny\bfseries, inner sep=1pt, minimum size=3.5mm] at ([xshift=-1.5mm, yshift=0mm]loss.north west) {3};
    
 % Connecting Arrows
    % \draw[->, primary, thick] (ctx.east) to[out=0, in=180] (pos.west);
    % \draw[->, primary, thick] (ctx.east) to[out=0, in=180] (neg.west);
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.2,0) |- (pos.west);
    \draw[->, primary, thick, rounded corners] (ctx.east) -- ++(0.2,0) |- (neg.west);
    \draw[->, accent, thick, rounded corners] (pos.east) -| ([xshift=2.4cm]loss.north);
    \draw[->, accent, thick, rounded corners] (neg.east) -| ([xshift=2.2cm]loss.north);

    % ==========================================
    % PANEL 3: GAIN DOWNSTREAM IMPACT
    % ==========================================
    \node[panel, minimum width=5.7cm, minimum height=4.5cm, anchor=south west] (p3) at (12.1, 0) {};
    \node[header] at (12.3, 4.3) {3. Downstream Impact};
    \node[subtext, text width=5.2cm] at (12.3, 3.8) {Higher precision translates into safer ranking and guided search.};
    
    % FPR Callout Badge
    \node[nodebox, draw=none, fill=accent!15, anchor=north, font=\scriptsize] at (14.95, 3.0) {\textbf{PRMBench FPR}: $\mathbf{69.3 \rightarrow 47.1}$};

    % Custom TikZ Graph (Clean and precise)
    \begin{scope}[shift={(13.0, 0.5)}]
        % Grid and Axes
        \draw[lightgray, very thin, dashed] (0,0) -- (4.0,0);
        \draw[lightgray, very thin, dashed] (0,0.6) -- (4.0,0.6);
        \draw[lightgray, very thin, dashed] (0,1.2) -- (4.0,1.2);
        \draw[lightgray, very thin, dashed] (0,1.8) -- (4.0,1.8);
        
        \draw[->, darkgray, thick] (0,0) -- (4.2,0) node[below, font=\tiny, xshift=-10mm, yshift=-1mm] {Solutions ($2^k$)};
        \draw[->, darkgray, thick] (0,0) -- (0,2.0) node[left, font=\tiny, rotate=90, yshift=2mm, xshift=-6mm] {AIME '24 Acc.};
        
        % Baseline Line
        \draw[bad, thick, densely dashed] (0,0.1) -- (0.8,0.1) -- (1.6,0.1) -- (2.4,0.1) -- (3.2,0.6) -- (4.0,0.6);
        \fill[bad] (0,0.1) circle (1.2pt) (0.8,0.1) circle (1.2pt) (1.6,0.1) circle (1.2pt) (2.4,0.1) circle (1.2pt) (3.2,0.6) circle (1.2pt) (4.0,0.6) circle (1.2pt);
        
        % PRISM Line
        \draw[good, thick] (0,0.6) -- (0.8,0.6) -- (1.6,0.6) -- (2.4,0.6) -- (3.2,1.2) -- (4.0,1.8);
        \fill[good] (0,0.6) circle (1.2pt) (0.8,0.6) circle (1.2pt) (1.6,0.6) circle (1.2pt) (2.4,0.6) circle (1.2pt) (3.2,1.2) circle (1.2pt) (4.0,1.8) circle (1.2pt);
        
        % Legend labels
        \node[font=\tiny\bfseries, text=bad, anchor=north west] at (2.4, 0.5) {PRM};
        \node[font=\tiny\bfseries, text=good, anchor=south east] at (3.3, 1.3) {PRISM};
    \end{scope}

    % ==========================================
    % INTER-PANEL ARROWS
    % ==========================================
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (5.75, 2.25) -- (6.0, 2.25);
    \draw[->, line width=1.5pt, draw=boxborder!80!gray] (11.8, 2.25) -- (12.05, 2.25);

\end{tikzpicture}

==> Figures/teaser_intro.tex <==
\begin{tikzpicture}[x=1cm,y=1cm,line cap=round,line join=round]
    \definecolor{teasernavy}{RGB}{31,59,91}
    \definecolor{teasertext}{RGB}{44,52,65}
    \definecolor{panelgold}{RGB}{251,241,212}
    \definecolor{panelblue}{RGB}{234,240,255}
    \definecolor{panelgreen}{RGB}{232,244,230}
    \definecolor{goodgreen}{RGB}{76,143,99}
    \definecolor{softgreen}{RGB}{231,244,234}
    \definecolor{badred}{RGB}{198,92,92}
    \definecolor{softred}{RGB}{252,236,234}
    \definecolor{softorange}{RGB}{252,239,214}
    \definecolor{accentblue}{RGB}{79,111,182}
    \definecolor{lightstroke}{RGB}{214,220,228}

    \tikzstyle{panel}=[rounded corners=0.22cm, draw=none, minimum height=4.45cm, minimum width=5.72cm]
    \tikzstyle{card}=[rounded corners=0.16cm, draw=lightstroke, line width=0.45pt, fill=white]
    \tikzstyle{pill}=[rounded corners=0.14cm, draw=none, inner xsep=5pt, inner ysep=2.2pt]

    \node[panel, fill=panelgold, anchor=south west] (leftpanel) at (0,0) {};
    \node[panel, fill=panelblue, anchor=south west] (midpanel) at (6.02,0) {};
    \node[panel, fill=panelgreen, anchor=south west] (rightpanel) at (12.04,0) {};

    \node[rounded corners=0.18cm, fill=teasernavy, text=white, anchor=south west,
          minimum width=17.76cm, minimum height=0.72cm, inner sep=0pt] at (0,4.73) {};
    \node[text=white, font=\bfseries\small, anchor=west] at (0.32,5.08)
        {\ours reduces false-positive overcredit so process rewards track sound reasoning instead of plausible mistakes.};

    \node[text=teasernavy, font=\bfseries\footnotesize, align=left, anchor=north west, text width=5.00cm] at (0.30,4.18)
        {1. Diagnose the failure mode};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=north west, text width=4.85cm] at (0.30,3.84)
        {Baseline overcredits a plausible mistake.};

    \node[card, anchor=south west, minimum width=5.10cm, minimum height=1.02cm] (goodcard) at (0.32,2.15) {};
    \fill[goodgreen] (0.32,2.15) rectangle (0.47,3.17);
    \node[text=goodgreen, font=\bfseries\scriptsize, align=left, anchor=north west] at (0.58,3.06) {Correct continuation};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=north west, text width=2.85cm] at (0.58,2.80)
        {Correct hypotenuse: $DF=10$, then solve for $DE$.};
    \node[pill, fill=softgreen, text=goodgreen, font=\bfseries\scriptsize, anchor=east] at (5.12,2.67) {reward $\uparrow$};

    \node[card, anchor=south west, minimum width=5.10cm, minimum height=1.16cm] (badcard) at (0.32,0.82) {};
    \fill[badred] (0.32,0.82) rectangle (0.47,1.98);
    \node[text=badred, font=\bfseries\scriptsize, align=left, anchor=north west] at (0.58,1.87) {Plausible but wrong};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=north west, text width=2.75cm] at (0.58,1.62)
        {Wrong hypotenuse: it uses $DE$ instead of $DF$.};
    \node[pill, fill=softorange, text=badred, font=\bfseries\scriptsize, anchor=east] at (5.12,1.52) {baseline: 0.91};
    \node[pill, fill=panelblue, text=accentblue, font=\bfseries\scriptsize, anchor=east] at (5.12,1.04) {\ours: 0.18};

    \node[pill, fill=softred, text=badred, font=\bfseries\scriptsize, anchor=west] at (0.34,0.36) {False positive $\rightarrow$ reward hacking};

    \draw[teasernavy, line width=0.9pt, -{Latex[length=2.2mm,width=1.8mm]}] (5.82,2.20) -- (5.98,2.20);
    \draw[teasernavy, line width=0.9pt, -{Latex[length=2.2mm,width=1.8mm]}] (11.84,2.20) -- (12.00,2.20);

    \node[text=teasernavy, font=\bfseries\small, anchor=west] at (6.32,4.10) {2. Train for reliable comparisons};
    \node[text=teasertext, font=\footnotesize, align=left, anchor=west, text width=5.02cm] at (6.32,3.55)
        {\ours turns existing step annotations into hard positive--negative comparisons and optimizes the relative margin directly.};

    \node[card, anchor=south west, minimum width=4.98cm, minimum height=0.82cm] (paircard) at (6.38,2.56) {};
    \node[circle, fill=accentblue!16, draw=accentblue!30, minimum size=0.42cm, inner sep=0pt] at (6.78,2.97) {\scriptsize $\pm$};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (7.12,3.05) {Matched step pairs};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=west, text width=3.75cm] at (7.12,2.72)
        {same prefix, correct next step vs. incorrect next step};

    \node[card, anchor=south west, minimum width=4.98cm, minimum height=0.82cm] (lookcard) at (6.38,1.48) {};
    \node[circle, fill=badred!14, draw=badred!28, minimum size=0.42cm, inner sep=0pt] at (6.78,1.89) {\scriptsize $\curvearrowright$};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (7.12,1.97) {Temporal lookahead hard negatives};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=west, text width=3.75cm] at (7.12,1.64)
        {reuse future steps as informative negatives without new labels};

    \node[card, anchor=south west, minimum width=4.98cm, minimum height=0.82cm] (losscard) at (6.38,0.40) {};
    \node[circle, fill=goodgreen!15, draw=goodgreen!30, minimum size=0.42cm, inner sep=0pt] at (6.78,0.81) {\scriptsize $\Delta$};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (7.12,0.89) {Step-Contrastive objective + curriculum};
    \node[text=teasertext, font=\scriptsize, align=left, anchor=west, text width=3.75cm] at (7.12,0.56)
        {widen the score margin, then introduce harder pairs gradually};

    \draw[accentblue, line width=0.7pt, -{Latex[length=1.8mm,width=1.5mm]}] (8.86,2.56) -- (8.86,2.30);
    \draw[accentblue, line width=0.7pt, -{Latex[length=1.8mm,width=1.5mm]}] (8.86,1.48) -- (8.86,1.22);
    \node[pill, fill=white, draw=accentblue!22, text=accentblue, font=\bfseries\scriptsize, anchor=west] at (6.38,3.78) {precision-first learning};

    \node[text=teasernavy, font=\bfseries\small, anchor=west] at (12.34,4.10) {3. Gain downstream reliability};
    \node[text=teasertext, font=\footnotesize, align=left, anchor=west, text width=5.02cm] at (12.34,3.55)
        {Better precision translates into safer ranking, better guided search, and stronger policy optimization.};

    \node[card, anchor=south west, minimum width=2.30cm, minimum height=1.05cm] at (12.36,2.42) {};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (12.62,3.12) {PRMBench FPR};
    \node[text=badred, font=\bfseries\small, anchor=west] at (12.60,2.64) {$69.3 \rightarrow 47.1$};
    \node[text=teasertext, font=\scriptsize, anchor=west] at (12.60,2.31) {$32.2\%$ reduction};

    \node[card, anchor=south west, minimum width=2.92cm, minimum height=1.05cm] at (14.82,2.42) {};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (15.08,3.12) {PRMScore};
    \node[text=goodgreen, font=\bfseries\small, anchor=west] at (15.06,2.64) {$65.5 \rightarrow 68.0$};
    \node[text=teasertext, font=\scriptsize, anchor=west] at (15.06,2.31) {better step ranking};

    \node[card, anchor=south west, minimum width=5.00cm, minimum height=1.48cm] at (12.36,0.34) {};
    \node[text=teasernavy, font=\bfseries\scriptsize, anchor=west] at (12.62,1.55) {Search consequence};
    \draw[gray!55, line width=0.65pt] (14.80,1.48) -- (13.72,0.74);
    \draw[gray!55, line width=0.65pt] (14.80,1.48) -- (15.88,0.74);
    \fill[teasernavy] (14.80,1.48) circle (0.055cm);
    \fill[goodgreen] (13.72,0.74) circle (0.055cm);
    \fill[badred] (15.88,0.74) circle (0.055cm);
    \node[text=goodgreen, font=\bfseries\scriptsize, anchor=north] at (13.72,0.61) {correct branch};
    \node[text=badred, font=\bfseries\scriptsize, anchor=north] at (15.88,0.61) {plausible wrong branch};
    \draw[goodgreen, line width=1.1pt, -{Latex[length=1.9mm,width=1.6mm]}] (14.36,1.25) -- (13.86,0.90);
    \draw[badred, densely dashed, line width=1.0pt, -{Latex[length=1.9mm,width=1.6mm]}] (15.22,1.25) -- (15.74,0.90);
    \node[pill, fill=softgreen, text=goodgreen, font=\bfseries\scriptsize, anchor=west] at (16.25,1.26) {\ours selects the right trace};
    \node[pill, fill=softred, text=badred, font=\bfseries\scriptsize, anchor=west] at (16.08,0.95) {baseline can be misled};
\end{tikzpicture}

==> sections/1.Introduction-old.tex <==
% \vspace{-2mm}
\section{Introduction}
% \vspace{-1mm}
% Large LLMs, including reasoning-oriented models, have shown tremendous capability; however, they suffer from shortcut behavior, often driven by reward hacking \cite{baker2025monitoring, denison2024sycophancy}. Shortcut behavior refers to the tendency of models to exploit superficial correlations or spurious cues that maximize reward signals without engaging in genuine reasoning. For instance, instead of carrying out a full algebraic derivation, a model might memorize input–output patterns for frequently seen problems, or rely on lexical overlap between the question and a candidate solution. In multi-step reasoning, models may also produce syntactically well-formed but semantically vacuous “reasoning chains” that appease automatic verifiers or judges while bypassing the actual logical computation. Such behaviors can inflate performance metrics without reflecting true reasoning ability.


% Large Reasoning models (LRMs) \citep{guo2025deepseek, shao2024deepseekmath, jaech2024openai} have achieved tremendous recent progress, demonstrating strong performance across mathematics, program synthesis, and planning tasks. However, they are typically trained using final-answer verification rewards (RLVR) \citep{lambert2024tulu}, which are inherently sparse. This sparsity leads to slow and inefficient convergence \citep{sun2025rl}, hard exploration challenges \citep{yue2025does}, and the emergence of incorrect reasoning behaviors \cite{zhang2025interplay}. Thus they can tolerate logically flawed traces that land on the correct outcome \citep{barkur2025deception, sun2025evaluation}. Process reward models (PRMs) are capable of training a better LRM by scoring \emph{intermediate} steps, offering dense supervision intended to shape safer, more faithful reasoning \citep{lightman2023let, chen2024alphamath, zhang2024rest}. However, current PRMs \citep{zhang2025lessons, wang2023math, khalifa2025process, zhao2025genprm}, both discriminative and generative suffer from several inherent limitations. 



% Reward models (RMs) are central to alignment pipelines for LLMs \citep{ouyang2022training}, as they provide generalization beyond the scope of limited human labeled preference data. Yet, when RMs assign high reward to incorrect responses (false positives), policies trained on them learn unintended shortcuts that amplify reward hacking. The challenge is particularly acute for process reward models (PRMs), which require step-level supervision of intermediate reasoning. Recent efforts, such as DeepSeek-R1 \citep{guo2025deepseek}, sidestep this challenge by using rule-based outcome rewards that evaluate only the final answer. While efficient, this approach produces unsafe or logically flawed reasoning chains that still land on the correct final output \citep{barkur2025deception, sun2025evaluation}. While it may learn to give correct final answer, emphasis on learning reasoning ability is reduced. To promote safer and correct reasoning, prior work has proposed PRMs that score intermediate steps and provide dense supervision signals \citep{lightman2023let, chen2024alphamath, zhang2024rest}. However, both discriminative PRMs \citep{zhang2025lessons, wang2023math} and recent generative PRMs \citep{khalifa2025process, zhao2025genprm} face persistent challenges.

% A key challenge in training effective reward models—whether PRMs or ORMs—is obtaining high-quality, balanced step-level or trajectory-level annotations. Acquiring such labels at scale without prohibitive cost remains an open problem. Importantly, the goal should not be limited to maximizing reward model accuracy, but rather to developing models that improve downstream alignment. A recurring issue in existing PRMs is their bias toward the majority class (see Table~\ref{tab:intro_SOTA_PRMs}), likely stemming from data imbalance and the use of point-wise loss during training. This bias often results in false positives, where the PRM assigns high reward to incorrect reasoning steps. Such errors directly undermine policy alignment and exacerbate reward hacking.

% In this work, we introduce a pairwise loss function which focus on learning both correct and incorrect steps. We construct training data from existing step-level annotations and apply simple augmentation strategies to further balance the dataset without incurring additional labeling costs. Our approach not only reduces false positives and improves PRM robustness but also yields significant gains in downstream alignment, as demonstrated on both guided beam search and best-of-N strategies. 

% The main contributions of our work are as follows. 

% \begin{itemize}
% \item  We provide both empirical and theoretical analyses of how false positive bias in PRMs leads to policy misalignment and reward hacking.
% \item  We propose a contrastive/pairwise loss framework plus techniques for balancing the training data (without needing new human labels) to reduce false positives.
% \item We design lightweight negative sample augmentation methods to produce more diverse “incorrect step” examples cheaply.
% \item  We evaluate PRMs capability on PRMBench, a recent PRM benchmark, and show improvements both in the accuracy / F1 of PRMs (especially negative/false-positive detection) and downstream alignment in guided beam search and Best-of-N settings. We see significant improvement in all benchmarks.
% \end{itemize}

% \textcolor{blue}{Souradip :  Reward hacking remains an extremely important issue in the context of fine-tuning frontier models with reinforcement learning, due to the potential for exploiting imperfections in learned reward proxies. While the majority of prior analyses have focused on reward hacking in the context of outcome reward models (ORMs), there is very limited research on process reward models (PRMs), making this an under-explored area. PRMs are especially vulnerable because they assign rewards to every intermediate step: a false positive (over-credit) at any step can both locally steer the search and globally accumulate across the trajectory. With additive aggregation, there is a compounding bias effect—so longer chains suffer much larger total distortion, leading to more severe reward hacking. This highlights why PRMs are particularly prone to reward hacking and underscores the importance of studying them in the context of post-training and alignment.
% 1.  \textbf{Motivation:} Reward Hacking in PRMs is Under-Explored \\
% Begin with a short paragraph introducing reward hacking as a central problem in alignment, especially in RLHF/post-training settings. Mention that prior work has mainly focused on Outcome Reward Models (ORMs).Emphasize that Process Reward Models (PRMs)—which assign scores at the step level—have not been analyzed from a reward hacking lens. \\
% 2. \textbf{Why PRMs are Especially Vulnerable} \\
% Explain that PRMs score every step, so: A false positive at any step can locally misguide decoding. And it accumulates globally i.e error compounding effect. - Plots and Visualizations \\
% 3. \textbf{Empirical Evidence of Reward Hacking in PRMs\\} 
% Step-Level Reward Hacking - Predicted reward vs. true reward at step level.
% Downstream Misalignment with Hacked PRM - Guided decoding and BoN selection using PRM vs. ground truth RM.. Highlight the gap between reward model accuracy and alignment performance. \\
% 4. \textbf{Alignment Performance is Important}\\
% Emphasize that the problem is not just about PRM accuracy and the key issue is when its used to train alignment, how it affects the downstream alignment performamnce.\\
% 5. Then highlight the issue of Reward hacking in the context through empiricala analysis - Need several key ablations
% 6. Show its due to the distribution of the data and the imbalance - Perform ablations to highlight this point. Show the data distribution imbalance clearly
% 7. Now, we want to mathematcally undersatant the issue-> BON analysis and effect of False positive and False negative -> highlight why FP being higher is crucial and critical \\ 
% 8. Mitigation strategiues :
% huge imbalance -> augmentation -> BT (call sth) -> balancing the data distribution
% step level distribution balancing. Show performance metrics
% FP rate is improving
% Eventually Step level; Controlled Decoding at Steps or MCTS works much better}


% ----------

% \sout{\textbf{Process supervision is powerful--but fragile.}Reasoning LLMs achieve strong results across mathematics, program synthesis, and planning, yet they remain vulnerable to \textit{reward hacking}: optimizing imperfect reward surrogates to produce persuasive but unsound chains of thought \citep{baker2025monitoring, denison2024sycophancy}. Outcome reward models (ORMs) trained from preferences \citep{ouyang2022training} score only final answers; they can}

Large Reasoning models \citep{guo2025deepseek, shao2024deepseekmath, jaech2024openai} have achieved tremendous recent progress, demonstrating strong performance across mathematics, program synthesis, and planning tasks. However, they are typically trained using final-answer verification rewards (RLVR) \citep{lambert2024tulu}, which are inherently sparse. This sparsity leads to slow and inefficient convergence \citep{sun2025rl}, hard exploration challenges \citep{yue2025does}, and the emergence of incorrect reasoning behaviors \cite{zhang2025interplay}.
Thus they can tolerate logically flawed traces that land on the correct outcome \citep{barkur2025deception, sun2025evaluation}. Process reward models (PRMs) are capable of training a better LRM by scoring \emph{intermediate} steps, offering dense supervision intended to shape safer, more faithful reasoning \citep{lightman2023let, chen2024alphamath, zhang2024rest}. However, current PRMs \citep{zhang2025lessons, wang2023math, khalifa2025process, zhao2025genprm}, both discriminative and generative suffer from several inherent limitations. 


\begin{figure}
    % \centering
    \includegraphics[width=0.5\textwidth, trim={360 50 50 40},
        clip]{Figures/example.pdf}
    \caption{An example illustrating reward hacking with the base PRM model, which does not occur with our trained PRM. This step-level reasoning example is generated by evaluating the policy using guided-beam search with the two different PRMs.}
    \label{fig:example}
    \vspace{-3mm}
\end{figure}

\textbf{Why Process supervision using PRMs is vulnerable.} Existing PRMs often \textit{overcredit} incorrect steps, yielding high false positive rates (Table~\ref{tab:intro_SOTA_PRMs}) that locally misguide decoding and, when aggregated across long chains, systematically bias search. This overcrediting of incorrect steps induces reward hacking in the downstream LLM policy. We attribute this issue to two primary factors.  First, step annotated corpora are imbalanced: correct steps are overrepresented even when most full solutions are incorrect (e.g., PRM800k; Table~\ref{tab:step_solution_distribution}) \citep{lightman2023let}. Second, most PRMs are trained with \emph{pointwise} cross entropy on step labels. Under imbalance and label noise, pointwise losses encourage majority class bias, inflating false positives. 
Thus, these PRMs are a direct risk factor for reward hacking during decoding or selection \citep{song2025prmbench} for the downstream LLM policy alignment, e.g. Best-of-N, Guided-Beam Search, where accurate ranking of the generated response is more important than absolute step correctness. 





\textbf{From PRM accuracy to downstream alignment.}
The ultimate goal is not a high average PRM accuracy but \emph{better reasoning behavior} when the PRM guides search (e.g., guided beam) or selection (e.g., Best of $N$). We therefore provide an analytic perspective that reveals a sharp asymmetry: in Best of $N$, the false positive rate $\alpha$ induces an \emph{asymptotic performance ceiling} equal to the classifier’s precision, while false negatives $\beta$ primarily slow convergence. Thus, reducing false positives is strictly more critical for trustworthy process supervision than merely improving recall. Eventually since PRMs are primarily used to improve policies under sparse reward settings, their true utility should be evaluated by downstream policy performance on decoding, selection, and ranking tasks.




\textbf{This work: comparison centered, label efficient PRMs.}
We introduce a simple, architecture agnostic recipe that requires no new human labels:
\textbf{(i)} convert existing step annotations into \emph{paired} positive–negative comparisons at matched contexts and train PRMs with a \emph{contrastive (pairwise) loss}, directly optimizing relative scores between correct and incorrect steps, with theoretical justification supported by empirical claims regarding this pairwise loss;
\textbf{(ii)} apply lightweight \emph{negative augmentation} by using future steps as negatives for earlier contexts, creating diverse, hard comparisons that counter overcredit; and
\textbf{(iii)} stabilize training with a small \emph{curriculum} over pair difficulty.
This shifts learning from pointwise accuracy to calibrated \emph{preference margins}, explicitly targeting the reduction of false positives.

\textbf{Empirical scope.}
On PRMBench \citep{song2025prmbench}, our method substantially lowers false positive rates and improves macro F1 for both discriminative and generative PRMs. When deployed to guide decoding (guided beam search) and selection (Best of $N$), the improved PRMs produce consistently higher downstream accuracy and robustness. Together with the Best of $N$ analysis, these results close the gap between reward model metrics and alignment outcomes.

\textbf{Contributions.} 
\setlength\itemsep{0pt}
\setlength\parsep{0pt}
\setlength\parskip{0pt}
\setlength\leftskip{0pt}
\begin{itemize}[leftmargin=*,topsep=0.1in]
\item \textbf{Analysis.} We formalize how step level overcredit compounds across trajectories and show that false positives impose an alignment ceiling in Best of $N$ selection, whereas false negatives mainly affect sample complexity.
\item \textbf{Method.} We propose a label efficient recipe—pairwise training on converted step annotations with lightweight negative augmentation and a simple curriculum—that directly optimizes comparative calibration and reduces false positives. We show both empirically and theoretically that pairwise losses are more effective for downstream policy decoding and selection.
\item \textbf{Results.} Across PRMBench and downstream guided decoding/Best of $N$, we observe substantial reductions in false positives, improved PRM macro F1 (especially on negatives), and stronger policy alignment. Our approach integrates cleanly with existing PRM pipelines \citep{lightman2023let, chen2024alphamath, zhang2024rest} without new human labels.
\end{itemize}


\textbf{Broader impact.}
Reducing PRM false positives decreases the risk that systems select fluent but incorrect chains, advancing safer, more trustworthy reasoning. Our findings argue for \emph{precision first} process supervision: train to \emph{compare} and calibrate, not merely to classify.


==> sections/Introduction-new.tex <==
\vspace{-8mm}

% \tableofcontents
\section{Introduction}\label{sec:intro} 
\vspace{-2mm}


\textcolor{blue}{Souradip - Flow of Intro
1. Whats PRM? Why its important whats the role of PRM? Why its so crucial - It improves credit asignment especially for large reasoning tasks where intermediate reward is crucial..
2. Issue in PRMs and Hidden Bias - However, there lies an important issue in the prms, the data imbalance. Explain brifely why data imbalance to this problem? Whats the key reason? Then end with resulting in high False positive rate
3. Policy-aware Evaluation of PRMs : Assymterical Impact of high FPR in downstream policy learning.Effect can be severe if there are more false positves
Thus the main question boils down to can we reduce false positive rate? but not at the cost of increasing FNR
We propose solution is in 2folds - 1. Training loss - Contrastive Loss
2. In order to generate data - data augmentation
3. Train using the contrastive loss - we use curriculum}


\textcolor{blue}{Souradip - Process Reward Models (PRMs) have become a central tool for improving large reasoning models because they provide step-level feedback, enabling better credit assignment in long reasoning tasks where final-answer rewards are too sparse. PRM evaluates intermediate reasoning steps and assigns rewards to partial solutions. This makes PRMs especially important for mathematical reasoning, program synthesis, and planning, where the quality of the final answer depends on many local decisions along the way.
%
However, in this paper, we identify a hidden but consequential bias in current PRMs: they systematically overcredit incorrect reasoning steps. A key reason is data imbalance. In process-supervision datasets, correct steps often appear much more frequently than incorrect steps, even when the full trajectory is ultimately wrong. This happens because a wrong solution may still contain many locally correct steps before the first critical mistake. As a result, the step-level training distribution becomes skewed toward positives. When PRMs are trained with standard pointwise classification losses on such data, they tend to inherit this positive bias, assigning high scores to fluent or plausible-looking steps even when they are incorrect. This produces a high false positive rate: many wrong steps are predicted as correct.
This false-positive bias is especially dangerous because PRMs are used inside downstream policy learning and inference-time search. If a correct step is mistakenly rejected, the system may need more samples or more search to recover. But if an incorrect step is mistakenly accepted, the policy can be actively pulled toward a flawed reasoning branch. In guided decoding, this can expand an incorrect partial solution. In Best-of-$N$ selection, it can choose a wrong solution that merely looks convincing to the PRM. In reinforcement learning, it can reinforce spurious reasoning patterns. Thus, false positives are not just local prediction errors; they become a direct mechanism for reward hacking.
This motivates a policy-aware view of PRM evaluation and mitigation. The goal is not simply to maximize average step-level accuracy, but to train PRMs that improve the policies using them. From this perspective, false positives and false negatives have asymmetric downstream effects. False negatives mainly reduce recall and slow search, while false positives can make incorrect reasoning appear rewarding and thereby mislead the policy itself. Therefore, the central question becomes: can we reduce the false positive rate of PRMs without substantially increasing the false negative rate?
Proposed solution - 
Contributions - }







\aak{Rewrite at the end} Large Reasoning models (LRMs) \citep{guo2025deepseek, shao2024deepseekmath, jaech2024openai} have achieved tremendous recent progress, demonstrating strong performance across mathematics, program synthesis, and planning tasks. However, they are typically trained using final-answer verification rewards (RLVR) \citep{lambert2024tulu}, which are inherently sparse. This sparsity leads to slow and inefficient convergence \citep{sun2025rl}, hard exploration challenges \citep{yue2025does}, and the emergence of incorrect reasoning behaviors \cite{zhang2025interplay}.
Thus they can tolerate logically flawed traces that land on the correct outcome \citep{barkur2025deception, sun2025evaluation}. Process reward models (PRMs) are capable of training a better LRM by scoring \emph{intermediate} steps, offering dense supervision intended to shape safer, more faithful reasoning \citep{lightman2023let, chen2024alphamath, zhang2024rest}. However, current PRMs \citep{zhang2025lessons, wang2023math, khalifa2025process, zhao2025genprm}, both discriminative and generative suffer from several inherent limitations. 




% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth, trim={360 50 50 42},
%         clip]{Figures/example.pdf}
%     \caption{Reward hacking induced by \emph{false-positive overcredit} in a baseline PRM. Under guided beam search, the baseline PRM assigns high reward to an incorrect intermediate step (a false positive), which locally steers the search toward a fluent but wrong chain. Our precision-first PRM reduces such overcrediting, preventing the same failure mode.}
%     \label{fig:example}
%     \vspace{-4mm}
% \end{figure}


\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth, trim={50 165 20 20}, clip]{Figures/intro_figure.pdf}
    \vspace{-3em}
    \caption{In this figure, we highlight the problem of reward hacking.  Reward hacking arises from the reward model’s bias toward predicting false positives, a bias that our trained model substantially reduces, as reflected in the lower FPR values (top-right) compared to the baseline. This effect is further illustrated in the reward distribution plot for label = 0 (top-left). For negative labels (dark blue), the baseline model assigns disproportionately high rewards. In contrast, our trained model shifts this distribution downward (silver), closer to the true reward of 0. This shift demonstrates that the trained PRM more accurately aligns negative labels with their intended reward, thereby reducing false-positive bias and alleviating reward hacking. Furthermore, when the trained PRM is used for downstream decoding in the LLM policy, it leads to significant performance improvements (bottom-right).}
    \label{fig:intro}
    \vspace{-3mm}
\end{figure*}

\textbf{Why process supervision via PRMs is vulnerable.}
In practice, many PRMs \emph{overcredit} incorrect intermediate steps, producing high false positive rates (Table~\ref{tab:intro_SOTA_PRMs}). A false positive is especially damaging at inference time: if an incorrect step is scored as ``good,'' it can steer decoding toward a flawed branch, and repeated overcredit across a long chain systematically biases search. In downstream use, this manifests as reward hacking by the guided policy (Figure~\ref{fig:example}).
We trace this vulnerability to two compounding factors.
\textbf{(1) Data imbalance:} step-annotated corpora are often heavily imbalanced: correct steps are overrepresented even when most full solutions are incorrect (e.g., PRM800k; Table~\ref{tab:step_solution_distribution})~\citep{lightman2023let}. \textbf{(2) Pointwise training:} most PRMs are trained with \emph{pointwise} cross-entropy on step labels. Under imbalance and label noise, pointwise objectives encourage majority-class bias, inflating false positives precisely. Consequently, these PRMs become unreliable rankers when used for policy \emph{selection} or \emph{search}---e.g., Best-of-$N$ and guided beam search---where the key requirement is to \emph{prefer correct traces over plausible but incorrect ones}, not merely to achieve high average step accuracy~\citep{song2025prmbench}.
\vspace{-1mm}

\textbf{From PRM accuracy to downstream alignment.}
The objective is not to maximize average PRM accuracy, but to improve reasoning behavior when the PRM guides \emph{decoding} (guided beam) or \emph{selection} (Best-of-$N$). 
We therefore analyze how PRM errors translate into downstream outcomes and uncover a sharp asymmetry: in Best-of-$N$, a false positive rate $\alpha$ induces an \emph{asymptotic performance ceiling} determined by the PRM's precision, while false negatives $\beta$ primarily slow convergence by increasing the number of samples required to find and recognize a correct solution. This implies a ``precision-first'' principle: reducing false positives is strictly more important for trustworthy process supervision than improving recall in isolation. Since PRMs are ultimately deployed to improve policies under sparse reward settings, their utility should be evaluated through downstream decoding, selection, and ranking performance, not just step-level metrics.



\vspace{-1mm}
\textbf{This work: \ours, comparison-centered and label-efficient PRMs.}
We introduce \ours~(\oursfull), an architecture-agnostic training recipe that requires no new human labels. \textbf{(i)} We convert existing step annotations into \emph{matched} positive--negative pairs and train PRMs with an \emph{Step-Contrastive} (pairwise) objective that directly optimizes the relative score of correct versus incorrect steps; we provide theoretical motivation and empirical evidence that this comparison-based training better supports ranking. \textbf{(ii)} We apply lightweight \emph{negative augmentation} by treating future steps as negatives for earlier contexts, creating diverse and hard comparisons that specifically counter overcredit. \textbf{(iii)} We stabilize optimization with a simple \emph{curriculum} over pair difficulty. Together, \ours shifts learning from pointwise label fitting to calibrated \emph{preference margins}, explicitly targeting reductions in false-positive overcredit.

\textbf{Empirical scope.}
On PRMBench \citep{song2025prmbench}, our method substantially lowers false positive rates and improves macro F1 for both discriminative and generative PRMs. When deployed to guide decoding (guided beam search) and selection (Best-of-$N$), the improved PRMs produce consistently higher downstream accuracy and robustness. Together with the Best-of-$N$ analysis, these results close the gap between reward model metrics and alignment.
\vspace{-1mm}


\textbf{Contributions.}
\vspace{-2mm}
\begin{itemize}[leftmargin=*,itemsep=0in,topsep=0in]
\item \textbf{Precision-first analysis.} We formalize how step-level \emph{overcredit} compounds across trajectories and prove a sharp asymmetry for Best-of-$N$: the false positive rate sets an \emph{asymptotic alignment ceiling} (via precision), whereas false negatives primarily increase sample complexity.
\item \textbf{\ours.} We introduce \ours~(\oursfull), a label-efficient, architecture-agnostic recipe that converts step labels into matched positive--negative pairs, optimizes a Step-Contrastive (pairwise) objective, and uses lightweight negative augmentation with a simple curriculum to reduce false-positive overcredit. We provide theoretical motivation and empirical evidence that comparison-based objectives better support downstream decoding and selection than pointwise training.
\item \textbf{Downstream-aligned gains.} On PRMBench and in guided decoding/Best-of-$N$, \ours substantially reduces false positives, improves macro F1 (especially on negative steps), and yields stronger policy alignment. The approach integrates cleanly with existing PRM pipelines~\citep{lightman2023let, chen2024alphamath, zhang2024rest} without new human labels.
\end{itemize}



\textbf{Broader impact.}
Reducing PRM false positives decreases the risk that systems select fluent but incorrect chains, advancing safer, more trustworthy reasoning. Our findings argue for \emph{precision first} process supervision: train to \emph{compare} and calibrate, not merely to classify.


